DaWin: Training-free Dynamic Weight Interpolation for Robust Adaptation

Adapting a pre-trained foundation model on downstream tasks should ensure robustness against distribution shifts without the need to retrain the whole model. Although existing weight interpolation methods are simple yet effective, we argue that their static nature limits downstream performance while achieving efficiency. In this work, we propose DaWin, a training-free dynamic weight interpolation method that leverages the entropy of individual models over each unlabeled test sample to assess model expertise, and compute per-sample interpolation coefficients dynamically. Unlike previous works that typically rely on additional training to learn such coefficients, our approach requires no training. Then, we propose a mixture modeling approach that greatly reduces inference overhead raised by dynamic interpolation. We validate DaWin on the large-scale visual recognition benchmarks, spanning 14 tasks across robust fine-tuning -- ImageNet and derived five distribution shift benchmarks -- and multi-task learning with eight classification tasks. Results demonstrate that DaWin achieves significant performance gain in considered settings, with minimal computational overhead. We further discuss DaWin's analytic behavior to explain its empirical success.

==> _figures/motiv_corr_reduced.tex <==
\vspace{-1em}
\begin{figure*}[t!]
\centering
    \includegraphics[width=.9\textwidth]{figure_files/motiv_corr_reduced.png}
    \vspace{-.5em}
\caption{\textbf{Correlation between entropy ratio and X-entropy ratio}. Results imply that the entropy ratio strongly correlates with the X-entropy ratio, except \texttt{FalseFalse} case, wherein given classifiers struggle to produce reliable predictions.
    }
    \vspace{-1em}
    \label{fig:motiv_corr}
\end{figure*}


==> _tables/mtl_runtime.tex <==
\begin{wraptable}{r}{0.33\textwidth}
%\begin{minipage}[]{0.34\textwidth}
\vspace{-1em}
% 
\caption{\textbf{Runtime comparison}. Wall-clock time on SVHN.}
\vspace{-0.75em}
\centering
\scriptsize
\begin{tabular}{@{}lc@{}}
\toprule
Method                & Wall-clock time \\ \midrule
Task Arithmetic          &  471.5 sec       \\
AdaMerging               &  1944.1 sec       \\
Layer-AdaMerging   &  2028.4 sec       \\
\rowcolor[HTML]{E1FFF5}
%
\textbf{\ours}           & 645.4 sec      \\ \bottomrule
%ours (K=1)
\end{tabular} \label{tab:runtime_mtl}
\vspace{-0.5em}
%\end{minipage}
\end{wraptable}

==> preamble.tex <==
\usepackage[cjk]{kotex}
\usepackage[font=small]{subcaption}
\usepackage[font=footnotesize]{subcaption}
\newcommand{\dy}[1]{\textcolor{RubineRed}{#1\xspace}}
\newcommand{\cd}[1]{\textcolor{Red}{#1\xspace}}

\usepackage[font=small]{caption}
\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} 
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

%\newcommand\ours{\textbf{\texttt{DaWin}}\xspace}
\newcommand\ours{\texttt{DaWin}\xspace}
\usepackage{enumerate}
